Influence of protostellar jets and HII regions on the formation and evolution of stellar clusters

Context. Understanding the conditions in which stars and stellar clusters form is of great importance. In particular the role that stellar feedback may have is still hampered by large uncertainties. Aims. We investigate the role played by ionising radiation and protostellar outflows during the formation and evolution of a stellar cluster. To self-consistently take into account gas accretion, we start with clumps of tens of parsecs in size. Methods. Using an adaptive mesh refinement code, we run magneto-hydrodynamical numerical simulations aiming at describing the collapse of massive clumps with either no stellar feedback or taking into account ionising radiation and/or protostellar jets. Results. Stellar feedback substantially modifies the protostellar cluster properties, in several ways. We confirm that protostellar outflows reduce the star formation rate by a factor of a few, although the outflows do not stop accretion and likely enough do not modify the final cluster mass. On the other hand, ionising radiation, once sufficiently massive stars have formed, efficiently expels the remaining gas and reduces the final cluster mass by a factor of several. We found that while HII radiation and jets barely change the distribution of high density gas, the latter increases, at a few places, the dense gas velocity dispersion again by a factor of several. As we are starting from a relatively large scale, we found that the clusters whose mass and size are respectively on the order of a few 1000 M and a fraction of parsec, present a significant level of rotation. Moreover we found that the sink particles which mimic the stars themselves, tend to have rotation axis aligned with the cluster large scale rotation. Finally, computing the classical Q parameter used to quantify stellar cluster structure, we infer that when jets are included in the calculation, [...]

==> Discussion.tex <==
\section{Discussion}
\label{section: discussion}




==> Macro_xvec.tex <==
% --- Macro \xvec
\makeatletter
\newlength\xvec@height%
\newlength\xvec@depth%
\newlength\xvec@width%
\newcommand{\xvec}[2][]{%
  \ifmmode%
    \settoheight{\xvec@height}{$#2$}%
    \settodepth{\xvec@depth}{$#2$}%
    \settowidth{\xvec@width}{$#2$}%
  \else%
    \settoheight{\xvec@height}{#2}%
    \settodepth{\xvec@depth}{#2}%
    \settowidth{\xvec@width}{#2}%
  \fi%
  \def\xvec@arg{#1}%
  \def\xvec@dd{:}%
  \def\xvec@d{.}%
  \raisebox{.2ex}{\raisebox{\xvec@height}{\rlap{%
    \kern.05em%  (Because left edge of drawing is at .05em)
    \begin{tikzpicture}[scale=1]
    \pgfsetroundcap
    \draw (.05em,0)--(\xvec@width-.05em,0);
    \draw (\xvec@width-.05em,0)--(\xvec@width-.15em, .075em);
    \draw (\xvec@width-.05em,0)--(\xvec@width-.15em,-.075em);
    \ifx\xvec@arg\xvec@d%
      \fill(\xvec@width*.45,.5ex) circle (.5pt);%
    \else\ifx\xvec@arg\xvec@dd%
      \fill(\xvec@width*.30,.5ex) circle (.5pt);%
      \fill(\xvec@width*.65,.5ex) circle (.5pt);%
    \fi\fi%
    \end{tikzpicture}%
  }}}%
  #2%
}
\makeatother

% --- Override \vec with an invocation of \xvec.
\let\stdvec\vec
\renewcommand{\vec}[1]{\xvec[]{#1}}
% --- Define \dvec and \ddvec for dotted and double-dotted vectors.
\newcommand{\dvec}[1]{\xvec[.]{#1}}
\newcommand{\ddvec}[1]{\xvec[:]{#1}}

==> Results_Q_old.tex <==
\subsection{Q parameter of the emerging clusters}
\label{section-sub: Q parameter of the emerging clusters}

In order to be able to characterise the emerging cluster in each of the four simulations, we computed the Q parameter. This quantity is commonly used to characterise such structures since it was introduced and developed by \citet{Cartwright2004, Cartwright2009}. This Q parameter is defined by:

\begin{equation}
    Q = \frac{\bar{l}_\text{MST}}{\bar{s}}
\end{equation}

\noindent
where $\bar{s}$ is the mean distance between stars, and $\bar{l}_\text{MST}$ is the mean edge length of the minimum spanning tree (MST) \citep[see e.g.][]{Boruvka1926,Kruskal1956,Prim1957,Gower1969}. A spanning tree is a set of straight lines connecting all the points of the sample without cycle. The MST is the unique spanning tree whose sum of edges is minimal. As the Q parameter has been introduced to describe observed clusters, $\bar{s}$ and $\bar{l}_\text{MST}$ are computed using the projected position of the stars in the plane of the sky. In order to be able to interpret the values of the Q parameter, \citet{Cartwright2004} computed the Q parameter for a set of fractal synthetic clusters, exhibiting radial concentration, homogeneous distribution, or sub-clusterisation. The values of $Q > 0.8$ corresponds to clusters with radial concentration, $Q \approx 0.8$ corresponds to clusters with homogeneous distribution, and $Q<0.8$ corresponds to clusters showing sub-clusterisation. All the clusters of this synthetic set were globally spherical. \citet{Cartwright2009} shows that for clusters with aspect ratios lower than 3 we can quit safely dismiss the effect of non-sphericity.


In our simulations we have access to the 3D positions of the stars. In order to be consistent with the observational method of computing the Q parameter, we projected our samples on 2D planes using the $x$, $y$, and $z$ axis of the simulation as lines of sight. In order to have enough sink particles in the cluster when we compute the Q parameter, we choose to begin at a time where approximately 300 sink particles are formed. In the four simulations, a lot of outliers are present. In order to minimise their effects on the Q parameter values, we resampled our set of stars by randomly choosing 90\% of the stars and we computed the Q parameter on this resampled set. We did this for a hundred randomly resampled sets, which lead us to a mean value and a standard deviation for the Q parameter over the resampled sets. The results for the three lines of sight are presented in Appendix \ref{annexe: Q parameter for different lines of sight} on Fig. \ref{figure: Q_stat_x_y_z}. As the results are similar for the three projections, we presented on Fig. \ref{figure: All_Q_stat_mean} the mean value of the Q parameter over the three projections. On this figure, the Q parameter is plotted over time for the four simulations represented by four distinct colours. The points represent the mean value of the Q parameter, while the colour filled areas represent the interval of the mean value $\pm 1 \sigma$, where the standard deviation $\sigma$ is obtained by $\sigma = \sqrt{\sigma_x^2+\sigma_y^2+\sigma_z^2}$. The first notable result is that two clear trends appear. On one hand, the two simulations that includes jets -- \sj{} and \sjrh{} -- show a similar evolution over time, while in the other hand, the two simulations that do not include jets -- \snj{} and \srh{} -- also show a similar trend, different from the first one. Both \sj{} and \sjrh{} show an increase in the Q parameter from 2.1 to \SI{2.7}{Myr}. At \SI{2.1}{Myr}, \sjrh{} has a Q parameter of about 0.6, which corresponds to a cluster exhibiting sub-clusterisation. Over time, it increases to about 0.8 which corresponds to a cluster with homogeneous distribution of the stars. At \SI{2.7}{Myr}, it drops from 0.8 to about 0.45, which corresponds again to a sub-clustered distribution, and then slowly increases from 0.45 to 0.6 at \SI{3.3}{Myr}. \sj{} has a Q parameter of about 0.8 at \SI{2.7}{Myr}, which corresponds to a cluster with homogeneous distribution. It increases to about 1 at \SI{2.7}{Myr}, which corresponds to a radially concentrated distribution of stars. Then it drops to 0.6 which corresponds to a sub-clustered distribution. The two simulations without jets, \snj{} and \srh{}, both have a Q parameter of about 0.6 at \SI{2.1}{Myr}, then it slowly decreases to 0.2 at \SI{2.8}{Myr}. At \SI{3}{Myr}, \snj{} it slowly increases from 0.2 to 0.3 at \SI{3.6}{Myr}. 

These results show two interesting points. The first one is that protostellar jets seem to play an important role in the structuring and distribution of stars in the cluster, while HII regions seem to only have a minor role in modifying this distribution. Looking at results presented in section \ref{section-sub: Global appearance of the emerging structures}, jets and HII regions have different impacts on the gas and the star cluster. Protostellar jets only have a minor influence on the gas appearance while having a major influence on the stars distribution in the cluster. Conversely, HII regions have a major role in shaping the gas but only have a minor impact on the distribution of stars in the cluster. The second interesting points is that the two simulations without protostellar jets -- \snj{} and \sjrh{} -- show a really low Q parameter. Those values for the Q parameter are lower than the typically observed values for the clusters with sub-clustered distributions. This implies that we should include protostellar jets to reproduce the observed values for the Q parameter. \textcolor{DarkMagenta}{Parler de la formation des sinks selon des arcs dans les simus sans jets, car c'est visiblement ce qui explique le Q parameter si bas. Attendons les retours de Marta?}


\noindent
\begin{figure}[hbtp] 
\includegraphics{All_Q_stat_mean.pgf}
\caption{The solid lines show the angular dispersion of the sink particles relatively to the mean angular direction, each colour corresponding to a different simulation. To consider only relevant sink particles, we selected the ones with a mass larger than \SI{0.07}{\Msun}. In comparison, the dotted lines show the angular dispersion of a set with the same cardinality than the set of sink particles at each time step, exhibiting random angular orientations. For times larger than \SI{2}{Myr}, the angular dispersion in the simulations is significantly lower than for a set of random orientations, implying that the sink particles have a preferred angular directions.}
\label{figure: All_Q_stat_mean}
\end{figure}

==> Theory.tex <==
\section{Theory}
\label{section: theory}


%\begin{equation}
%\left. \bm{\sigma_O} \right| _{_{\mathcal{R}}} = \sum_i m_i \bm{OM_i} \times \frac{\d \bm{OM_i}}{\d t}
%\label{moment 0}
%\end{equation}

















